Saturation Physics on the Energy Frontier

Saturation physics is expected to be relevant at sufficiently small parton momentum fractions $x$ in high-energy proton- (or deuteron-)ion collisions at RHIC and the LHC. Accordingly, these collisions provide the best available testing ground for the saturation model. However, producing precise numerical predictions from the model is a complicated task; the state of the art in this area involves next-to-leading order QCD calculations, which are difficult to do numerically. Here I'll review recent progress in extracting numerical predictions from saturation models and matching them to experimental results.

==> plotfiles/proceedings-plotdata.tex <==
\pgfplotstablesort[row sep=\\]\brahmsdAuhiY{
% http://www4.rcf.bnl.gov/brahms/WWW/publication-data/RdA-letter/newdau_eta3.dat
% h^- from d+Au collisions (eta=3.2)
pt          ptlo                pthi                yield       staterr         syserr         \\
% pt[GeV/c] pt bin low[GeV/c]   pt bin high[GeV/c]  yield       stat error      sys error (?)
0.25        0.2                 0.3                 2.01147     0.0258206       0.3017205      \\
0.35        0.3                 0.4                 1.45906     0.0174999       0.218859       \\
0.45        0.4                 0.5                 0.933742    0.0114546       0.1400613      \\
0.55        0.5                 0.6                 0.466025    0.00760817      0.06990375     \\
0.65        0.6                 0.7                 0.293151    0.00555747      0.04397265     \\
0.75        0.7                 0.8                 0.142542    0.00358952      0.0213813      \\
0.85        0.8                 0.9                 0.085915    0.00174568      0.01288725     \\
0.95        0.9                 1                   0.0559974   0.00123521      0.00839961     \\
1.09        1                   1.2                 0.0233523   0.000140574     0.00467046     \\
1.29        1.2                 1.4                 0.0104938   8.29051e-05     0.00209876     \\
1.49        1.4                 1.6                 0.00506653  4.97884e-05     0.001013306    \\
1.69        1.6                 1.8                 0.00246804  3.15367e-05     0.000493608    \\
1.89        1.8                 2                   0.00120714  1.93553e-05     0.000241428    \\
2.13        2                   2.3                 0.000459623 9.66696e-06     6.89434e-05    \\
2.55        2.3                 2.9                 0.000124681 3.42328e-06     1.870215e-05   \\
3.31        2.9                 4                   1.22812e-05 7.80291e-07     1.84218e-06    \\
}

\pgfplotstablesort\atlaspPb{
% charged hadrons from pPb collisions at CM rapidity
pT           -2.25       -1.75        0.00        1.75
0.175      34.8999     31.3004     29.3542         nan
0.225      25.9138     23.2411      21.474         nan
0.275      19.2415     17.7784     16.4267         nan
0.325      14.5014     13.3988     12.5657         nan
0.375      11.0929     10.4032     9.75634         nan
0.425      8.87311     8.38357     7.57509     8.24432
0.475      7.06238     6.60685     6.05924     6.66031
0.525       5.5107     5.24557     4.77511     5.27491
0.600      4.21545     4.16476     3.68918     4.03507
0.675      3.32207     3.25779     3.01009     3.19574
0.825       1.7257     2.08441     1.89747     2.00453
0.950      1.40107     1.14921     1.30785     1.04128
1.075     0.857286    0.879092    0.824432     0.77317
1.200      0.60875    0.615011    0.576771     0.54902
1.375     0.432267     0.43026    0.409559    0.372827
1.600     0.227914    0.230258     0.21918    0.194633
1.875       0.1238    0.126949    0.119056     0.10416
2.125    0.0615011   0.0627532   0.0618451    0.051873
2.375          nan   0.0378301   0.0367318   0.0301288
2.725    0.0216949   0.0222467   0.0224755   0.0179835
3.275   0.00836796    0.009336   0.0092009  0.00736198
3.775   0.00363579  0.00401634   0.0041185   0.0031987
4.250   0.00140237  0.00154915   0.0016611  0.00130947
4.750  0.000696663 0.000781122  0.00083757 0.000680221
5.500  0.000378418 0.000418026 0.000454957 0.000371325
6.500  9.91182e-05 0.000106281 0.000126477 0.000103741
7.500  3.93863e-05 4.52705e-05  5.3341e-05 4.35356e-05
8.500  1.76301e-05 2.02138e-05 2.31761e-05 1.80001e-05
9.500   8.6288e-06 9.53196e-06  1.1686e-05 9.30413e-06
11.275 3.16712e-06 3.36246e-06 4.41885e-06 3.79002e-06
13.750 9.39113e-07 1.08478e-06 1.29092e-06 1.19276e-06
18.750 1.57384e-07 1.76464e-07 2.47356e-07 1.87406e-07
}
\pgfplotstablesort\atlaspPblab{
% charged hadrons from pPb collisions at pseudorapidity in lab frame
pT           2.25       1.50      -0.50      -2.25
0.175   31.917777  27.786385  26.058815  26.721762
0.225   24.415699  22.559378  20.232792  20.542651
0.275   18.309908  17.429038  15.709305  15.177801
0.325   14.006276  13.398766  12.318785  11.269797
0.375   10.608389  10.506927   9.612225   8.620900
0.425    8.785450   8.530427   7.688726   7.210692
0.475    6.992615   6.857347   6.242369   5.682543
0.525    5.429261   5.324236   4.919435   4.456087
0.600    4.215430   4.195880   3.857680   3.425667
0.650    3.322062   3.306655   3.055251   2.713100
0.725    2.657285   2.644961   2.468238   2.127535
0.775    2.157413   2.115679   2.013896   1.727316
0.850    1.725693   1.743450   1.626961   1.395442
0.900    1.401066   1.415483   1.327477   1.138576
0.975    1.137506   1.149210   1.093923   0.924394
1.050    0.870142   0.870415   0.836803   0.686379
1.175    0.608750   0.621147   0.591264   0.494700
1.300    0.425880   0.436715   0.415705   0.344378
1.425    0.302413   0.314758   0.304108   0.243329
1.550    0.221230   0.230260   0.221368   0.184298
1.675    0.161840   0.165957   0.165188   0.133492
1.800    0.118394   0.123226   0.124494   0.099120
1.925    0.090566   0.094263   0.093826   0.075447
2.125    0.058815   0.062134   0.063715   0.049979
2.375    0.033908   0.036904   0.037283   0.029391
2.625    0.020441   0.022247   0.022476   0.017630
2.875    0.012695   0.014024   0.014596   0.011004
3.125    0.007884   0.008840   0.009201   0.007253
3.375    0.005045   0.005741   0.006065   0.004734
3.625    0.003325   0.003784   0.004119   0.003183
3.875    0.002192   0.002570   0.002797   0.002140
4.250    0.001270   0.001474   0.001678   0.001284
4.750    0.000647   0.000743   0.000850   0.000667
5.250    0.000331   0.000400   0.000469   0.000366
5.750    0.000188   0.000222   0.000268   0.000210
6.500    0.000087   0.000105   0.000126   0.000103
7.500    0.000036   0.000042   0.000053   0.000043
8.475    0.000016   0.000019   0.000023   0.000018
9.500    0.000007   0.000009   0.000012   0.000009
11.250   0.000003   0.000003   0.000005   0.000004
13.750   0.000001   0.000001   0.000001   0.000001
18.750   0.000000   0.000000   0.000000   0.000000
}

\def\readdata#1#2#3#4{
 \def\filenamepattern##1{#1}
 \expandafter\pgfplotstablesort\csname #4himu\endcsname{\filenamepattern{#3}}
 \expandafter\pgfplotstablesort\csname #4lomu\endcsname{\filenamepattern{#2}}
}
\readdata{plotfiles/brahms-dAu-mu#1-rcBKL01.Y32.summary.dat}{10}{50}{brahmsrcBKB}
\readdata{plotfiles/atlas-pPb-mu#1-rcBKL01.Y175.summary.dat}{10}{100}{atlasrcBKB}


==> plotfiles/proceedings-plotsetup.tex <==
\usepackage{graphicx}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{physics}
\usepackage{siunitx}
%\usepackage{drawproton}
\pgfplotsset{compat=1.10}
\usetikzlibrary{calc}
%\usetikzlibrary{detectorcs}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{external}
\usetikzlibrary{fadings}
\usetikzlibrary{fit}
% \usetikzlibrary{intersections}
\usetikzlibrary{patterns}
\usetikzlibrary{positioning}
\usetikzlibrary{shadows}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{shapes.symbols}
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{fillbetween}

% BEGIN tikz styles
\tikzset{momentum/.style={blue}}

\tikzset{quark/.style={draw,postaction={decorate},decoration={markings,mark=at position .55 with {\arrow{>}}}}}
\tikzset{antiquark/.style={draw,postaction={decorate},decoration={markings,mark=at position .55 with {\arrow{<}}}}}
\tikzset{lepton/.style={draw,postaction={decorate},decoration={markings,mark=at position .55 with {\arrow{>}}}}}
\tikzset{antilepton/.style={draw,postaction={decorate},decoration={markings,mark=at position .55 with {\arrow{<}}}}}
\tikzset{gluon/.style={decorate,decoration={coil,amplitude=1mm,segment length=2mm}}}
\tikzset{small gluon/.style={decorate,decoration={coil,amplitude=0.4mm,segment length=0.8mm}}}
\tikzset{photon/.style={decorate,decoration={snake,amplitude=2pt,segment length=5pt}}}
\tikzset{weak/.style={decorate,decoration={zigzag,amplitude=3pt,segment length=5pt}}}

\newlength\baryonlinespacing
\setlength\baryonlinespacing{5pt}
\tikzset{baryon/.style={to path={-- (\tikztotarget) \tikztonodes},
  execute at begin to={
   \draw ($(\tikztostart)!\baryonlinespacing!90:(\tikztotarget)$)--($(\tikztotarget)!\baryonlinespacing!-90:(\tikztostart)$);
   \draw[quark] (\tikztostart)--(\tikztotarget);
   \draw ($(\tikztostart)!\baryonlinespacing!-90:(\tikztotarget)$)--($(\tikztotarget)!\baryonlinespacing!90:(\tikztostart)$);
  }}
 }
\tikzset{right half baryon/.style={to path={-- (\tikztotarget) \tikztonodes},
  execute at begin to={
   \draw[quark] (\tikztostart)--(\tikztotarget);
   \draw ($(\tikztostart)!\baryonlinespacing!-90:(\tikztotarget)$)--($(\tikztotarget)!\baryonlinespacing!90:(\tikztostart)$);
  }}
 }
\tikzset{left half baryon/.style={to path={-- (\tikztotarget) \tikztonodes},
  execute at begin to={
   \draw ($(\tikztostart)!\baryonlinespacing!90:(\tikztotarget)$)--($(\tikztotarget)!\baryonlinespacing!-90:(\tikztostart)$);
   \draw[quark] (\tikztostart)--(\tikztotarget);
  }}
 }
\tikzset{nucleus/.style={to path={-- (\tikztotarget) \tikztonodes},
  execute at begin to={
   \draw ($(\tikztostart)!1.5\baryonlinespacing!90:(\tikztotarget)$)--($(\tikztotarget)!1.5\baryonlinespacing!-90:(\tikztostart)$);
   \draw ($(\tikztostart)!1.2\baryonlinespacing!90:(\tikztotarget)$)--($(\tikztotarget)!1.2\baryonlinespacing!-90:(\tikztostart)$);
   \draw ($(\tikztostart)!0.9\baryonlinespacing!90:(\tikztotarget)$)--($(\tikztotarget)!0.9\baryonlinespacing!-90:(\tikztostart)$);
   \draw ($(\tikztostart)!0.3\baryonlinespacing!90:(\tikztotarget)$)--($(\tikztotarget)!0.3\baryonlinespacing!-90:(\tikztostart)$);
   \draw[quark] (\tikztostart)--(\tikztotarget);
   \draw ($(\tikztostart)!0.3\baryonlinespacing!-90:(\tikztotarget)$)--($(\tikztotarget)!0.3\baryonlinespacing!90:(\tikztostart)$);
   \draw ($(\tikztostart)!0.9\baryonlinespacing!-90:(\tikztotarget)$)--($(\tikztotarget)!0.9\baryonlinespacing!90:(\tikztostart)$);
   \draw ($(\tikztostart)!1.2\baryonlinespacing!-90:(\tikztotarget)$)--($(\tikztotarget)!1.2\baryonlinespacing!90:(\tikztostart)$);
   \draw ($(\tikztostart)!1.5\baryonlinespacing!-90:(\tikztotarget)$)--($(\tikztotarget)!1.5\baryonlinespacing!90:(\tikztostart)$);
  }}
 }
\tikzset{blob/.style={ellipse,minimum height=0.8cm,minimum width=0.3cm}}
\tikzset{interaction/.style={ellipse,minimum height=0.3cm,minimum width=0.3cm}}

\tikzset{
 xq2shading/.style={
  rounded corners=5pt,
  drop shadow,
  preaction={
   fill=white,
   draw=black,
   line width=0.2pt
  },
  opacity=0.15,
  top color=red!70!magenta,
  bottom color=cyan,
  middle color=red!70!magenta!50!cyan!30!white,
  shading angle=45
 }
}

\tikzset{on shell cross/.pic={\draw[thick] (0,0) +(45:.2) -- +(45:-.2) +(-45:.2) -- +(-45:-.2);}}

\tikzfading[name=dual fade,top color=transparent!100,bottom color=transparent!100,middle color=transparent!0]

\colorlet{partondist}{green!60!black}
\colorlet{gluondist}{red!80!black}
\colorlet{fragmentation}{cyan!60!black}
\colorlet{kinfactor}{blue!40!red!70!black}
% END tikz styles


% BEGIN externalization configuration (except for the actual call to \tikzexternalize)
\tikzset{external/only named=true}
\tikzsetexternalprefix{generated-figures/}
% END externalization configuration

% BEGIN conversion factors
% 1.3 converts from yields for pi- only to yields of all negative hadrons
\pgfmathsetmacro\brahmshadronconversionfactor{1.3*1770/2400}
% STAR measures neutral pions
\pgfmathsetmacro\starhadronconversionfactor{1770/2210}
% factor of 2 because we calculate for negative particles but the data are for both charges
% factor of 1.2 to account for the production of kaons and other non-pions
% factor of 1/1.2 to account for the ratio of sigma_total to Sperp
\pgfmathsetmacro\alicehadronconversionfactor{1.2*2*1830/2100}
\pgfmathsetmacro\atlashadronconversionfactor{1.2*2*1830/2100}
% END conversion factors

\newcommand\fixedcoupling[1]{1}
\newcommand\runningcoupling[1]{pi/(2.25*(ln(greater(#1,1)*#1+notgreater(#1,1)*1) - ln(0.0588)))/0.2}
\newcommand\coupling[1]{\runningcoupling{#1}}

\newcommand\setplotshift[2]{\expandafter\newcommand\csname plotshift-#1\endcsname{#2}}
\newcommand\plotshift[1]{\csname plotshift-#1\endcsname}

\newcommand\resultplot[2]{
 { % begin a TeX scope
  \expandafter\pgfplotstablevertcat\expandafter\himudata\csname #2himu\endcsname
  \expandafter\pgfplotstablevertcat\expandafter\lomudata\csname #2lomu\endcsname
  \addplot[#1,result plot line,name path=hi mu] table {\himudata};
  \addplot[#1,result plot line,forget plot,name path=lo mu] table {\lomudata};
  \addplot[#1,result plot fill] fill between[of=hi mu and lo mu];
 }
}

% BEGIN styles
\pgfplotsset{
 result axis/.style={
  % needs to be nearly transparent, otherwise it obscures the result plot fill
  axis background/.style={fill=gray!40,fill opacity=0.1},
  ymin=1e-6, % just a default
  xlabel={$p_\perp [\si{GeV}]$},
  ylabel={$\frac{\dd[3]{N}}{\dd{\eta}\dd[2]{\pperp}} \bigl[\si{GeV^{-2}}\bigr]$},
  legend style={cells={anchor=west}},
  legend columns=1,
  % explanation of flags at http://tex.aspcode.net/view/635399273629833626198028/using-nan-values-in-pgfplots
  y filter/.code={
   \let\tmpy=\pgfmathresult
   \pgfmathparse{rawy}
   \let\tmprawy=\pgfmathresult
   \pgfmathfloatgetflagstomacro\tmprawy\flags
   \ifnum\flags=3 % nan (missing data)
    \def\pgfmathresult{}
   \else
    \ifnum\flags=0 % zero
     \def\pgfmathresult{-40}
    \else
     \ifnum\flags=2 % negative
      \def\pgfmathresult{-40}
     \else
      \let\pgfmathresult=\tmpy
     \fi
    \fi
   \fi
  }
 },
 data plot/.style={
  black,
  only marks,
  mark=*,
  mark size=3pt,
  every mark/.append style={draw=gray!30!white,fill=black,line width=0.5pt}
%   error bars/y dir=both,
%   error bars/y explicit,
%   error bars/error bar style={line width=2pt,no markers}
 },
 ghost data plot/.style={
  gray,
  mark=*,
  mark size=1pt,
  every mark/.append style={fill=gray!30!white}
 }
}

% data plot table layout
\pgfplotsset{
 brahms data/.style={
  table/.cd,
  x index=0,
  y=yield,
  y error expr={(\thisrow{staterr} + \thisrow{syserr})}
 },
 star data/.style={
  table/.cd,
  x=pt,
  y expr={(\thisrow{xsec}/\starsigmainel)},
  y error expr={((\thisrow{staterr} + \thisrow{syserr})/\starsigmainel)}
 },
 alice y0 data/.style={
  table/.cd,
  x=pt,
  y=yield0,
  y error plus expr={(\thisrow{stat0plus} + \thisrow{sys0plus})},
  y error minus expr={(\thisrow{stat0minus} + \thisrow{sys0minus})}
 },
 alice y055 data/.style={
  table/.cd,
  x=pt,
  y=yield055,
  y error plus expr={(\thisrow{stat055plus} + \thisrow{sys055plus})},
  y error minus expr={(\thisrow{stat055minus} + \thisrow{sys055minus})}
 },
 alice y105 data/.style={
  table/.cd,
  x=pt,
  y=yield105,
  y error plus expr={(\thisrow{stat105plus} + \thisrow{sys105plus})},
  y error minus expr={(\thisrow{stat105minus} + \thisrow{sys105minus})}
 },
 cms y0 data/.style={
  table/.cd,
  x=pT,
  y expr={(\thisrow{yield}/(2*pi*\thisrow{pT}))},
  y error plus expr={(\thisrow{errplus}/(2*pi*\thisrow{pT}))},
  y error minus expr={(\thisrow{errminus}/(2*pi*\thisrow{pT}))}
 },
 atlas y0 data/.style={
  table/.cd,
  x=pT,
  y=0.00
 },
 atlas y175 data/.style={
  table/.cd,
  x=pT,
  y=1.75
 }
}

% calculated curve styles
\pgfplotsset{
 LO/.style={
  /pgfplots/result plot fill/.style={
   /tikz/draw=none,
   /tikz/preaction={
    /tikz/fill=#1,
    /tikz/fill opacity=0.2
   },
   /tikz/pattern=crosshatch,
   /tikz/pattern color=#1,
   /pgfplots/area legend
  },
  /pgfplots/result plot line/.style={
   /tikz/draw=#1,
   /tikz/mark=x,
   /tikz/mark size={0.5pt},
   /tikz/mark options={fill=#1},
   /pgfplots/forget plot
  }
 },
 NLO/.style={
  /pgfplots/result plot fill/.style={
   /tikz/draw=none,
   /tikz/preaction={
    /tikz/fill=#1,
    /tikz/fill opacity=0.3,
   },
   /tikz/pattern=grid,
   /tikz/pattern color=#1,
   /pgfplots/area legend
  },
  /pgfplots/result plot line/.style={
   /tikz/draw=#1,
   /tikz/mark=x,
   /tikz/mark size={0.5pt},
   /tikz/mark options={fill=#1},
   /pgfplots/forget plot
  }
 },
 exact/.style={
  /pgfplots/result plot fill/.style={
   /tikz/draw=none,
   /tikz/preaction={
    /tikz/fill=#1,
    /tikz/fill opacity=0.2,
   },
   /tikz/pattern=crosshatch dots,
   /tikz/pattern color=#1,
   /pgfplots/area legend
  },
  /pgfplots/result plot line/.style={
   /tikz/draw=#1,
   /tikz/mark=x,
   /tikz/mark size={0.5pt},
   /tikz/mark options={fill=#1},
   /pgfplots/forget plot
  }
 },
 extra/.style={
  /pgfplots/result plot fill/.style={
   /tikz/draw=none,
   /tikz/fill=#1,
   /tikz/fill opacity=0.5,
   /pgfplots/area legend
  },
  /pgfplots/result plot line/.style={
   /tikz/draw=#1,
   /tikz/mark=x,
   /tikz/mark size={0.5pt},
   /tikz/mark options={fill=#1},
   /pgfplots/forget plot
  }
 },
 rcBK LO/.style={
  LO=cyan!50!blue
 },
 rcBK NLO/.style={
  NLO=red
 },
 rcBK exact/.style={
  exact=green!50!black!70!purple
 },
 rcBK extra/.style={
  extra=green!35!black
 },
 BK LO/.style={
  LO=blue
 },
 BK NLO/.style={
  NLO=magenta
 },
 MV LO/.style={
  LO=green!50!black
 },
 MV NLO/.style={
  NLO=orange
 },
 MV extra/.style={
  extra=magenta!70!white
 },
 GBW LO/.style={
  LO=green
 },
 GBW NLO/.style={
  NLO=brown
 },
 GBW extra/.style={
  extra=cyan
 }
}

% calculated curve table layout
\pgfplotsset{
 xsec LO/.default=1,
 xsec LO/.style={
  table/x=pT,
  table/y expr={#1*\thisrow{lo-mean}}
 },
 xsec LO plus sigma/.default=1,
 xsec LO plus sigma/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}+\thisrow{lo-stddev})}
 },
 xsec LO minus sigma/.default=1,
 xsec LO minus sigma/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}-\thisrow{lo-stddev})}
 },
 xsec LO upper error estimate/.default=1,
 xsec LO upper error estimate/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}+\thisrow{lo-errbound})}
 },
 xsec LO lower error estimate/.default=1,
 xsec LO lower error estimate/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}-\thisrow{lo-errbound})}
 },
 xsec NLO/.default=1,
 xsec NLO/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}+\coupling{\thisrow{mu2}}*\thisrow{nlo-mean})}
 },
 xsec NLO plus sigma/.default=1,
 xsec NLO plus sigma/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}+\thisrow{lo-stddev}+\coupling{\thisrow{mu2}}*(\thisrow{nlo-mean}+\thisrow{nlo-stddev}))}
 },
 xsec NLO minus sigma/.default=1,
 xsec NLO minus sigma/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}-\thisrow{lo-stddev}+\coupling{\thisrow{mu2}}*(\thisrow{nlo-mean}-\thisrow{nlo-stddev}))}
 },
 xsec NLO upper error estimate/.default=1,
 xsec NLO upper error estimate/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}+\thisrow{lo-errbound}+\coupling{\thisrow{mu2}}*(\thisrow{nlo-mean}+\thisrow{nlo-errbound}))}
 },
 xsec NLO lower error estimate/.default=1,
 xsec NLO lower error estimate/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}-\thisrow{lo-errbound}+\coupling{\thisrow{mu2}}*(\thisrow{nlo-mean}-\thisrow{nlo-errbound}))}
 },
 xsec Lqg/.default=1,
 xsec Lqg/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}+\coupling{\thisrow{mu2}}*(\thisrow{nlo-mean}+\thisrow{lq-mean}+\thisrow{lg-mean}))}
 },
 xsec Lqg plus sigma/.default=1,
 xsec Lqg plus sigma/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}+\thisrow{lo-stddev}+\coupling{\thisrow{mu2}}*(\thisrow{nlo-mean}+\thisrow{nlo-stddev}+\thisrow{lq-mean}+\thisrow{lq-stddev}+\thisrow{lg-mean}+\thisrow{lq-stddev}))}
 },
 xsec Lqg minus sigma/.default=1,
 xsec Lqg minus sigma/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}-\thisrow{lo-stddev}+\coupling{\thisrow{mu2}}*(\thisrow{nlo-mean}-\thisrow{nlo-stddev}+\thisrow{lq-mean}-\thisrow{lq-stddev}+\thisrow{lg-mean}-\thisrow{lq-stddev}))}
 },
 xsec Lqg upper error estimate/.default=1,
 xsec Lqg upper error estimate/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}+\thisrow{lo-errbound}+\coupling{\thisrow{mu2}}*(\thisrow{nlo-mean}+\thisrow{nlo-errbound}+\thisrow{lq-mean}+\thisrow{lq-errbound}+\thisrow{lg-mean}+\thisrow{lq-errbound}))}
 },
 xsec Lqg lower error estimate/.default=1,
 xsec Lqg lower error estimate/.style={
  table/x=pT,
  table/y expr={#1*(\thisrow{lo-mean}-\thisrow{lo-errbound}+\coupling{\thisrow{mu2}}*(\thisrow{nlo-mean}-\thisrow{nlo-errbound}+\thisrow{lq-mean}-\thisrow{lq-errbound}+\thisrow{lg-mean}-\thisrow{lq-errbound}))}
 },
 brahms/.style={},
 brahms xsec LO/.style={
  xsec LO=\brahmshadronconversionfactor,
  brahms
 },
 brahms xsec NLO/.style={
  xsec NLO=\brahmshadronconversionfactor,
  brahms
 },
 brahms xsec Lqg/.style={
  xsec Lqg=\brahmshadronconversionfactor,
  brahms
 },
 star/.style={},
 star xsec LO/.style={
  xsec LO=\starhadronconversionfactor,
  star
 },
 star xsec NLO/.style={
  xsec NLO=\starhadronconversionfactor,
  star
 },
 star xsec Lqg/.style={
  xsec Lqg=\starhadronconversionfactor,
  star
 },
 alice/.style={},
 alice xsec LO/.style={
  xsec LO=\alicehadronconversionfactor,
  alice
 },
 alice xsec NLO/.style={
  xsec NLO=\alicehadronconversionfactor,
  alice
 },
 alice xsec Lqg/.style={
  xsec Lqg=\alicehadronconversionfactor,
  alice
 },
 cms/.style={},
 cms xsec LO/.style={
  xsec LO=\cmshadronconversionfactor,
  cms
 },
 cms xsec NLO/.style={
  xsec NLO=\cmshadronconversionfactor,
  cms
 },
 cms xsec Lqg/.style={
  xsec Lqg=\cmshadronconversionfactor,
  cms
 },
 atlas/.style={},
 atlas xsec LO/.style={
  xsec LO=\atlashadronconversionfactor,
  atlas
 },
 atlas xsec NLO/.style={
  xsec NLO=\atlashadronconversionfactor,
  atlas
 },
 atlas xsec Lqg/.style={
  xsec Lqg=\atlashadronconversionfactor,
  atlas
 },
}

% END styles

